TrafficLLM: Enhancing Large Language Models for Network Traffic Analysis with Generic Traffic Representation

Machine learning (ML) powered network traffic analysis has been widely used for the purpose of threat detection. Unfortunately, their generalization across different tasks and unseen data is very limited. Large language models (LLMs), known for their strong generalization capabilities, have shown promising performance in various domains. However, their application to the traffic analysis domain is limited due to significantly different characteristics of network traffic. To address the issue, in this paper, we propose TrafficLLM, which introduces a dual-stage fine-tuning framework to learn generic traffic representation from heterogeneous raw traffic data. The framework uses traffic-domain tokenization, dual-stage tuning pipeline, and extensible adaptation to help LLM release generalization ability on dynamic traffic analysis tasks, such that it enables traffic detection and traffic generation across a wide range of downstream tasks. We evaluate TrafficLLM across 10 distinct scenarios and 229 types of traffic. TrafficLLM achieves F1-scores of 0.9875 and 0.9483, with up to 80.12% and 33.92% better performance than existing detection and generation methods. It also shows strong generalization on unseen traffic with an 18.6% performance improvement. We further evaluate TrafficLLM in real-world scenarios. The results confirm that TrafficLLM is easy to scale and achieves accurate detection performance on enterprise traffic.

==> 6-discussion/discussion.tex <==


\textbf{Computation Overhead}.
Given the constraints on time, performance, and computational resources in network analysis, achieving a balance is essential when deploying LLM-based network systems. For LLM applications, model quantization techniques~\cite{xu2023survey} are extensively used to address the challenges of deploying LLMs in real-world environments. These techniques can be incorporated into \textsf{TrafficLLM} to minimize overhead. We utilized quantization to reduce \textsf{TrafficLLM}'s bit-width to 4 bits, resulting in a 4-fold reduction in model size and a 3.5-fold decrease in memory consumption. Additionally, \textsf{TrafficLLM} can reach lower detection latency than existing ML models with negligible degradation in accuracy using quantization techniques (see Appendix~\ref{efficiency}).

\vspace{0.1cm}
\noindent \textbf{LLM Hallucination}.
Hallucinations~\cite{JiLFYSXIBMF23} can negatively impact the generation results of LLMs, thereby reducing the accuracy of traffic analysis. Furthermore, the implicit and non-textual nature of network knowledge makes constructing Retrieval-Augmented Generations (RAGs)~\cite{lewis2020retrieval} as straightforwardly as in natural language tasks challenging. To address this, we evaluate the hallucinations in \textsf{TrafficLLM} and mitigate them through the use of different sampling strategies (see Appendix~\ref{hallucination}). \textsf{TrafficLLM} can effectively mitigate the issue through adjustments to the sampling parameters.

\vspace{0.1cm}
\noindent \textbf{Robustness of \textsf{TrafficLLM}}.
More complex network scenarios and adversarial attacks may affect the robustness of ML-based models. However, existing experiments in extensive tasks, concept drift scenarios, and real-world deployment have shown that TrafficLLM has the scalability to extend to other complex network environments. This effectiveness is largely attributed to the TrafficLLM's robust representation learning ability for different text and traffic data (see Appendix~\ref{representation}). Furthermore, we assess potential adversarial attacks to \textsf{TrafficLLM} with jailbreak instructions and traffic adversarial samples. Our findings indicate that regular jailbreak attacks~\cite{YuLLCXZ24} are ineffective due to \textsf{TrafficLLM}’s architectural design with dual-stage tuning. This ensures a strict gating mechanism for task execution. In addition, similar to existing work~\cite{LuLPL25, LiZBYLSW23}, we can also fine-tune \textsf{TrafficLLM} with adversarial samples to enhance the accuracy under adversarial attacks at the traffic level.

% MadryMSTV18, KurakinGB17, abs-2211-12681, MetzenGFB17
